Trajectory and Policy Aware Sender Anonymity in Location Based Services

We consider Location-based Service (LBS) settings, where a LBS provider logs the requests sent by mobile device users over a period of time and later wants to publish/share these logs. Log sharing can be extremely valuable for advertising, data mining research and network management, but it poses a serious threat to the privacy of LBS users. Sender anonymity solutions prevent a malicious attacker from inferring the interests of LBS users by associating them with their service requests after gaining access to the anonymized logs. With the fast-increasing adoption of smartphones and the concern that historic user trajectories are becoming more accessible, it becomes necessary for any sender anonymity solution to protect against attackers that are trajectory-aware (i.e. have access to historic user trajectories) as well as policy-aware (i.e they know the log anonymization policy). We call such attackers TP-aware. This paper introduces a first privacy guarantee against TP-aware attackers, called TP-aware sender k-anonymity. It turns out that there are many possible TP-aware anonymizations for the same LBS log, each with a different utility to the consumer of the anonymized log. The problem of finding the optimal TP-aware anonymization is investigated. We show that trajectory-awareness renders the problem computationally harder than the trajectory-unaware variants found in the literature (NP-complete in the size of the log, versus PTIME). We describe a PTIME l-approximation algorithm for trajectories of length l and empirically show that it scales to large LBS logs (up to 2 million users).

==> abstract.tex <==
We consider Location-based Service (LBS) settings, where a LBS provider logs the requests sent by mobile device users over a period of time and later wants to publish/share these logs. Log sharing can be extremely valuable for advertising, data mining research and network management, but it poses a serious threat to the privacy of LBS users.
Sender anonymity solutions prevent a malicious attacker from inferring the interests of LBS users by associating them with their service requests after gaining access to the anonymized logs. With the fast-increasing adoption of smartphones and the concern that historic user trajectories are becoming more accessible, it becomes necessary for any sender anonymity solution to protect against attackers that are trajectory-aware (i.e. have access to historic user trajectories) as well as policy-aware (i.e they know the log anonymization policy). We call such attackers TP-aware.

This paper introduces a first privacy guarantee against TP-aware attackers, called {\em TP-aware sender k-anonymity}. It turns out that there are many possible TP-aware  anonym\-izations for the same LBS log, each with a different utility to the consumer of the anonym\-ized log. The problem of finding the optimal TP-aware anonymization is investigated. We show that trajectory-awareness renders the problem computationally harder than the traj\-ectory-unaware variants found in the literature (NP-complete in the size of the log, versus PTIME). We describe a PTIME l-approx\-imation algorithm for trajectories of length $l$ and empirically show that it scales to large LBS logs (up to 2 million users).


\eat{
Sender anonymity in Location-based Services refers to hiding the identity of a 
mobile device user who sends requests to the Location-Based Service (LBS) 
provider. The best-studied identity protection measure in this context is known 
as {\it sender k-anonymity}. We show that the prior solutions provide sender 
k-anonymity to the LBS requests only against naive attackers who have no 
knowledge of the user movements over a period of time (trajectory) and the 
anonymization policy that is in use. We strengthen the privacy guarantee to 
defend against a stronger class of attackers who know the 
user trajectories (\emph{trajectory-aware}) and have complete knowledge of the
anonymization policy (\emph{policy-aware}). We call it
\emph{trajectory-aware policy-aware} (\emph{TP}-aware) sender k-anon\-ymity.

In this paper we show how this novel privacy guarantee is provided in an 
\emph{offline} scenario, when a LBS provider logs the LBS requests sent by 
its users over a period of time and later wants to publish/share these logs. 
While these logs can be extremely valuable for advertising, data 
mining research and network management, we show they pose a serious threat
to the anonymity of the LBS users. We describe a method to anonymize these 
LBS request logs and preserve trajectory-aware policy-aware sender 
k-anonymity in the offline scenario. We show that finding the optimum offline 
policy that provides trajectory-aware policy-aware k-anonymity is 
\emph{NP-Hard}. Hence, we describe a novel bounded approximation algorithm 
%that computes an anonymization policy whose cost is guaranteed to be within $l$ 
%times that of optimum policy for user trajectories of length $l$. We 
and empirically show the effectiveness of this approximation algorithm for 
anonymizing large sizes of data (up to 2 million users). 
}
